Driving-Signal Aware Full-Body Avatars

We present a learning-based method for building driving-signal aware full-body avatars. Our model is a conditional variational autoencoder that can be animated with incomplete driving signals, such as human pose and facial keypoints, and produces a high-quality representation of human geometry and view-dependent appearance. The core intuition behind our method is that better drivability and generalization can be achieved by disentangling the driving signals and remaining generative factors, which are not available during animation. To this end, we explicitly account for information deficiency in the driving signal by introducing a latent space that exclusively captures the remaining information, thus enabling the imputation of the missing factors required during full-body animation, while remaining faithful to the driving signal. We also propose a learnable localized compression for the driving signal which promotes better generalization, and helps minimize the influence of global chance-correlations often found in real datasets. For a given driving signal, the resulting variational model produces a compact space of uncertainty for missing factors that allows for an imputation strategy best suited to a particular application. We demonstrate the efficacy of our approach on the challenging problem of full-body animation for virtual telepresence with driving signals acquired from minimal sensors placed in the environment and mounted on a VR-headset.

==> dumpster.tex <==
\begin{comment}
\subsubsection{Dynamic Formulation}
The second scenario happens when arbitrary parts of the control signal can be missing. 
%
Again, in this case, control signal $\bc$ contains two types of variables: 
those which are observed, and those which are not, either due to noise / occlusions, 
or due to a limited capture setup.
%
For example, for a human body, observed control variables would correspond
to \textit{unoccluded joints}, and unobserved variables would represent
occluded joints, as well as the values which are not captured by joint 
angles, such as state of clothing and certain muscle activations.
 
Let $\bb \in { 0, 1 }^{N_c}$ be binary masks that indicate to which of the two
sets each variable $\bc_{i}$ belongs to: $\bb_i = 1$ if the variable $\bc_i$ 
is observed, and $\bb_i = 0$ otherwise. 
%
Given $\bb$ and \textit{incomplete} controls $\tilde{\bc}$ we want to obtain the
distribution over the controls $q_{\bc}(\bc | \bb, \tilde{\bc})$, which 
acts as a prior for unobserved values, and is used to fill in the missing values,
in particular by sampling from this distribution.
\TB{I am not sure if this will lead to a model that would produce reasonable
uncertainty, currently trying this out}.
% 
A naive way of defining $q_{\bc}$ would be a Gaussian with diagonal covariance, 
with both parameters produced by a neural network conditioned on $\tilde{\bc}$, $\bb$. 
%
During training, we typically have access to uncorrupted controls, which 
we can artificially corrupt, and then obtain samples $\bc \sim q_{\bc}$ 
with the reparameterization trick.
%
During inference, now we have the flexibility to use $q_{\bc}$ in a variety
of ways: for example, simply taking the mean of the distribution
for the missing values, or, producing multiple samples and then 
using them to produce a visual representation of uncertainty (e.g.
render multiple semi-transparent explanations for the missing parts).
\end{comment}

% old
\begin{comment}
The baseline approach is the “standard” body avatar which models articulated motion + pose-dependent deformations. A naive approach to extend this model would be to expand this model by introducing embeddings that capture deformations that do not stem from body pose. But the resulting representation is not ideal as it mixes together information between different modalities. This causes generalization problems, in particular for animation, since it is not feasible to collect all possible combinations of configurations even at train time, and currently seems infeasible to reliably produce both of those things with commodity capture devices.

To solve this problem, we propose a following three-step approach. 
First, we identify as many factors which can be reliably estimated during online tracking, and build highly accurate models for acquiring these measurements. This comprises a set of partially-overlapping components: body poses (in the form of joint angles), hand articulations (in the form of joint angles), and facial expression (in the form of latent embeddings). Ground truth for these measurements are acquired using a system for multiview capture, and a model for real-time detection and tracking from minimal cameras are learned from that data.
Second, we build a per-frame (static) representation where all of the measured factors are separated from all other factors in the latent space of a generative model of the entire body. Examples of non-measured factors include body dynamics and clothing deformations. This is achieved with a disentangling method: a variant of MINE for now. 
Lastly, we build a temporal model, the goal of which is to generate plausible sequences of the unmeasured factors that take into account some “hand-chosen/random” initial state as well as the temporal dynamics of the measured factors. The idea is that even though on per-frame basis these types of factors are now independent, their changes over time are still very correlated. For example, there can be multiple states of clothing with exactly the same initial pose, but the way those clothing states will change as the person moves, clearly depend on those pose changes (as well as the initial clothing configuration). 

Method summary:
Partition representation into face, body, hands and the rest (clothing etc), and estimate (non-exclusive) parameters for each. Is this data preparation only?
Learn a disentangled representation that allows the generation of realistic static images of fully bodies by mix-and-matching the different elements (face embeddings, joint angles for body and hands, clothing), demonstrating better generalization of body model
Learn a temporal model that conditions on some elements (face + body) and produces consistent temporal estimates of the others (clothing), demonstrating our model can generate realistic dynamics based on animation signals. 


\subsection{Local Representations}
\label{sec:method:local-representations}

The main idea is to introduce inductive bias in the model to encourage the local control over body parts. The motivation for this is better generalization to unseen poses, as we effectively increase the number of samples that the model observes. This should also help model to avoid learning spurious correlations.


\subsection{“Multi-decoder” model }
Here we essentially use multiple decoders, each defined on a subregion which is controlled by a subset of
pose parameters (this is similar to STAR, but the mapping there is linear). Those are then joined together 
in a learned way. In practice, for the UV-based architecture it means that we have to define multiple 
different UV-mappings (one per region), so it seems reasonable to use mesh-conv-like architecture instead. 


\subsection{Region penalty disentangling}
Use pre-defined regions of influence for multiple subsets of joints (e.g. based on skinning weights) to penalize changes outside of those regions. In practice it means running decoder additional time on perturbed outputs: to get a perturbed input we choose a single factor and shuffle its value within the mini-batch, while keeping all others fixed. The difference between the output of the decoder on perturbed vs non perturbed is then used as a penalty.

\subsection{Estimating shading}
A large percent of artifacts is coming from the ambiguity between shading and albedo. 
\end{comment}



% Done:
% \begin{itemize}
%     \item Pre-train "pose imputation" model - with 2 fingers as driving signal - produces reasonable samples.
%     \item Initial version with full decoder \href{{http://hewen.sb.facebook.net:8082/visualize/home/timurb/trash/hand_disentangling/videos/side_by_side_codec_combined_new_16-20_kl0.01_mine100_v3_samples.mp4}}{video}
% \end{itemize}

% In progress:
% \begin{itemize}
%     \item Improving the quality
%     \item Alternative imputation techniques (matrix effects?)
% \end{itemize}



% \subsection{Old}

% In each, we want to demonstrate that the model
% can produce high-fidelity outputs for different levels
% of missing input data. 

% Intuitively, for the bodies we expect to see that it
% helps with capturing clothes / muscle activations, 
% for faces probably some non-pose-dependent deformations 
% that are missing from some the restricted views (think of
% headset views which cover a small amount),
% for hands - some of the deformations which are not 
% in the sparsified set of keypoints (think of driving
% only by fingertips).


% Data preparation:
% \begin{itemize}
% \item Preselect Mugsy sequences with interesting  with artificial Argent views (Jason and Shih-En) 
% \TB{No need to prepare artificial argent views, we can proceed with partial keypoints?}
% \item Can we capture Autumn in the wild, potentially running openpose on both (Shih-En?)
% \item Check if we already have Autumn in different clothing (Chenglei)
% \item Choose an interesting sequence for the hands (Takaaki)
% \end{itemize}



% Random thoughts:
% \begin{itemize}
%     \item it would be nice to produce a video grid where on
%     one axis we vary the amount of data, and on another method / disentanglement settings
%     \item we should find a pose representation which makes it easier to drop
%     parts of the signals, and which is not necessarily global
%     \item what do we do about model robustness to the inputs - training
%     with 
%     \item locality-based disentangling: should it be a part of the 
%     narrative or just a way to make it work better.
%     \item image-based generative model for a talk show?
%     \item we need to find a reasonable set of "missing data imputation"
%     techniques.
% \end{itemize}



% We want to demonstrate that disentangling and temporal modeling improve generalization. 
% The ultimate application is driving an avatar with a set of sparse signals, potentially unreliable or missing of observations.
% Build and validate generalization of body, face and clothing representations 
% Demonstrate the effects of disentangling and its benefits. 
% Demonstrate the effects of temporal modeling.
% Demonstrate effectiveness on unseen sequences 
% Ablation studies: enable / disable disentangling, enable / disable temporal, architecture choices. 

% \subsection{Baselines}
% A rough list of models that makes sense to consider (e.g. in ablation studies) and what we expect to see:

% \begin{itemize}
%     \item Pose-only: 
% we cannot hope that it captures the facial expressions, or any clothing state (if it does it means overfitting)
%     % \item Latent-space-only: 
%     \item Latent+pose:\CW{we may want to show this version on both body and hand sequence. One is on the body for the test sequence to show that with disentanglement it creates sharper results. The other we could show on the hand by optimizing the conditioning signal with respect to the 3d keypoint constraint to show that without disentanglement, the missing part is constrained to be heavily correlated with conditioning signal, while we are able to sample the missing parts.} \TB{I like this.}
%     \item Explicit disentangling pose + latent via MINE / dropout:
%     \item Locality-based disentangling:
%     \item Joint disentangling:
% \end{itemize}


% \subsection{Evaluating Drivability}
% Initially: we can do either latent optimization, or encoder-only optimization to see how well the decoder works on test sequences. Fitting done via IR-based loss (single-view geometry + texture reconstruction?). 

